A Declarative Goal-oriented Framework for Smart Environments with LPaaS

Smart environments powered by the Internet of Things aim at improving our daily lives by automatically tuning ambient parameters (e.g. temperature, interior light) and by achieving energy savings through self-managing cyber-physical systems. Commercial solutions, however, only permit setting simple target goals on those parameters and do not consider mediating conflicting goals among different users and/or system administrators, and feature limited compatibility across different IoT verticals. In this article, we propose a declarative framework to represent smart environments, user-set goals and customisable mediation policies to reconcile contrasting goals encompassing multiple IoT systems. An open-source Prolog prototype of the framework is showcased over two lifelike motivating examples.

==> src/tmp.tex <==
Suppose that is a sunny morning in winter and user {\tt\small u1} sets the brightness of her room to 0 and the temperature to 18$^{\circ}$C. On the contrary, user {\tt\small 3} sets the temperature at 28$^{\circ}$. Assume that the two rooms share the air conditioning system but not the lighting system. Meanwhile, user {\tt\small u4} sets the temperature and brightness of {\tt\small room2}, which she is not authorised to handle. Finally, users {\tt\small u2} and {\tt\small u8} are both in the {\tt\small commonRoom\_E} with the same goal for the light but different goals for the temperature (respectively 23$^{\circ}$C and 18$^{\circ}$C).

\begin{Verbatim}[fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}]
season(winter).

user(u1, [room_E_1, commonRoom_E, commonRoom_W]).
set(u1, room_E_1, roomLight, 0).
set(u1, room_E_1, roomTemp, 18).

user(u3, [room_E_3, commonRoom_E, commonRoom_W]).
set(u3, room_E_3, roomTemp, 28).

user(u4, [room_E_4, commonRoom_E, commonRoom_W]).
set(u4, room_E_2, roomLight, 0).
set(u4, room_E_2, roomTemp, 18).

user(u2, [room_W_1, commonRoom_E, commonRoom_W]).
set(u2, commonRoom_W, commonRoomLight, 255).
set(u2, commonRoom_W, commonRoomTemp, 23).

user(u8, [room_W_4, commonRoom_E, commonRoom_W]).
set(u8, commonRoom_W, commonRoomLight, 255).
set(u8, commonRoom_W, commonRoomTemp, 18).
\end{Verbatim}
\noindent
for each room the result of the mediation phase with the application of global policies is:
\begin{Verbatim}[fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}]
[(room_E_1,roomLight,100),
(room_E_1,roomTemp,18),
(room_E_3,roomTemp,22),
(commonRoom_W,commonRoomLight,255),
(commonRoom_W,commonRoomTemp,20.5)]
\end{Verbatim}
\noindent
where {\tt\small roomLight} of {\tt\small room\_E\_1} is bounded on 100 because it is the minimum bound for the light in the East wing, while the {\tt\small roomTemp} is within the bounds. Meanwhile, {\tt\small roomTemp} of {\tt\small room\_E\_3} is bounded to 22 the maximum temperature allowed in winter. Instead in {commonRoom\_W} the temperature is the average of the two requests because it is within the boundaries and also the light because we are in the West wing and it is sunny so the maximum bound is 255, the goal of both users. Finally, the goals of user {\tt\small u4} are ignored because is not authorised to interact with {\tt\small room\_E\_2}.
%
\hfill$\diamond$

%Returning to the example of the \textit{Smart Building} we can imagine a possible policy to mediate conflicts between users: make the average between all requests and then compare the average with company directives. Company directives consider in which wing the zone is located, and information such as the season and the weather to limit the minimum and maximum value that can be assumed by each property. For the sake of brevity, we will not explain how averaging is carried out\footnote{see: LINK} but we will focus on writing company policies:

%In this case, regardless of the wing, the minimum and maximum temperatures allowed vary according to the seasons, trying to be as eco-friendly as possible. On the contrary, the brightness depends both on the wing and in the case of the west wing (the one most exposed to the sun) also on the weather to adapt to the external brightness. Regarding the generation of the actions, we can assume a simple policy like dividing the workload equally among all the possible actuators.

\noindent
the actions, given the desired states computed above, to be carried out will be:
\begin{Verbatim}[fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}]
  [(acCommonRoom_W, 20.5),  
  (biglightCommonRoom_W_1, 127.5),  
  (biglightCommonRoom_W_2, 127.5),  
  (acOdd_E, 22),  
  (heater, 100),  
  (biglightRoom_E_1, 50),  
  (smalllightRoom_E_1, 50)] 
 \end{Verbatim}
 \noindent
where the temperature of {commonRoom\_W} is managed only by {\tt\small acCommonRoom\_W} and the light is implemented by two main light which equally divide the goal. Meanwhile, {\tt\small acOdd\_E} is the air conditioning system shared by room 1 and 3 and is setted to the maximum of the two goals (18 and 22) and also in {\tt\small room\_E\_1} the {\tt\small heater} is working. Finally, the small and big light work together to implement the goal.
%
\hfill$\diamond$

%Suppose that users 2, 5 and 8 are all in the east common room, each with their own goals:
%\begin{Verbatim}[fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}]
%set(u2, commonRoom_E, commonRoomLight, 100).
%set(u2, commonRoom_E, commonRoomTemp, 18).
%set(u5, commonRoom_E, commonRoomLight, 100).
%set(u5, commonRoom_E, commonRoomTemp, 23).
%set(u8, commonRoom_E, commonRoomLight, 255).
%set(u8, commonRoom_E, commonRoomTemp, 28).
%\end{Verbatim}
%\noindent
%the target state, obtained from the mediation and conflict resolution policies will be:
%\begin{Verbatim}[fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}]
%[(commonRoom_E,commonRoomLight,151.7),
%(commonRoom_E,commonRoomTemp,22)]
%\end{Verbatim}
%\noindent
%the actions to be carried out will, therefore, be:
%\begin{Verbatim}[fontsize=\footnotesize, frame=single, framesep=1mm, framerule=0.1pt, rulecolor=\color{gray}]
%[(acCommonRoom_E, 22),  
%(biglightCommonRoom_E_1, 75.8),
%(biglightCommonRoom_E_2, 75.8)]
%\end{Verbatim}
%
